The Oxford Road Boundaries Dataset

In this paper we present the Oxford Road Boundaries Dataset, designed for training and testing machine-learning-based road-boundary detection and inference approaches. We have hand-annotated two of the 10 km-long forays from the Oxford Robotcar Dataset and generated from other forays several thousand further examples with semi-annotated road-boundary masks. To boost the number of training samples in this way, we used a vision-based localiser to project labels from the annotated datasets to other traversals at different times and weather conditions. As a result, we release 62605 labelled samples, of which 47639 samples are curated. Each of these samples contains both raw and classified masks for left and right lenses. Our data contains images from a diverse set of scenarios such as straight roads, parked cars, junctions, etc. Files for download and tools for manipulating the labelled data are available at: oxford-robotics-institute.github.io/road-boundaries-dataset

==> reviews.tex <==
Reviewer 1 of IV 2021 submission 520
-	Authors could have elaborated more on their
network’s [15] result. Further metrics, what partitioning
they used, etc. would allow for new methods to compare to
their result
-	Table one contains “Manual” and “Automatic”
annotation methods. This is not explained in either the
caption or the text.I assume the Automatic corresponds to
the second traversal projection method but some
clarification would be useful.
-	“enabling automatic partitioning of the raw
training data into two classes”: how? This algorithmic part
– net output to binary decisions is not explained in
detail. Please add explanation

Reviewer 2 of IV 2021 submission 520
1) I'd love to see a similar approach to leading benchmarks
in machine vision (KITTI, Cityscapes, ...) that also
outline a set of evaluation metrics to be used with the
dataset. Particularly, as the problem of road boundary
estimation is not a standard machine vision problem, some
guidelines on how to properly evaluate approaches are
highly desirable. This could be done via the dataset
webpage, although I did not see on the webpage (yet). 

3) As a last point, I was wondering whether the annotation
error in the images could be quantified. By annotating
mainly in Lidar data, followed by a projection into the
camera space, spatial and temporal registration errors will
happen, even with the proposed temporal warping of point
clouds onto the timestamps of camera images. Given that
road boundaries are static, my feeling is that these errors
only have a minor impact (if the ego-motion estimation of
the vehicle is "good"). Nevertheless, I would like to see
some comments on that. 
